PokerSkill: LLMs Can Play Expert-Level Poker without Training or Solvers

Poker is a landmark challenge for artificial intelligence. The dominant approach relies on equilibrium solvers built on counterfactual regret minimization, requiring millions of core-hours of training. Large Language Models (LLMs) possess extensive poker knowledge but perform far below solver-based agents when asked to play directly. Traditional rule-based poker agents are interpretable and training-free, but their strategic ceiling remains far below equilibrium play. We introduce \textbf{PokerSkill}, a training-free and solver-free framework that bridges this gap by using detailed rule-based poker skills as a structured action-grounding interface for LLMs. A deterministic context engine analyzes the current state and retrieves only the relevant fragments from a layered skill library, which is entirely designed by human poker experts, constraining the LLM's choice to reasonable actions. Against GTOWizard, a state-of-the-art GTO benchmark, GPT-5.5 XHigh with PokerSkill achieves $-57 \pm 21$ mbb/hand, Claude Opus 4.6 achieves $-80 \pm 29$ mbb/hand and Claude Opus 4.7 achieves $-87\pm 64$ mbb/hand, reducing losses by 49--61\% compared to default-prompt baselines and outperforming the strong bot Slumbot. Our key finding is that rule-based skills alone do not constitute a strong strategy, and LLMs alone cannot play well, but their combination yields an agent that requires neither training nor solver access yet competes with systems built on millions of core-hours of computation. To our knowledge, this is the first demonstration of an LLM achieving competitive performance in a complex imperfect-information game without game-specific training or solver queries. Code is available at https://github.com/lbn187/PokerSkill.

==> figures/latex_includes.tex <==
% === Fig. 1: PokerSkill overview ===
\begin{figure*}[t]
    \centering
    \includegraphics[width=0.95\textwidth]{figures/overview.pdf}
    \caption{PokerSkill converts raw HUNL game states into compact, decision-relevant abstractions before prompting the LLM. A deterministic context engine computes board texture, hand strength, action-line scenario, position, SPR, and ATT/DEF budgets; these labels select only the relevant skill layers (P1--P5 Blocker). The LLM therefore acts as a bounded strategic reasoner rather than an unstructured poker simulator, and its output is validated before execution.}
    \label{fig:overview}
\end{figure*}

% === Fig. 2: Main GTOWizard results ===
\begin{figure}[t]
    \centering
    \includegraphics[width=0.48\textwidth]{figures/gtowizard_main_results.pdf}
    \caption{Performance of PokerSkill and LLM baselines against GTOWizard, reported in bb/100 with AIVAT evaluation. Llama 3.3 70B + PokerSkill scores $-6.1 \pm 6.6$ bb/100, GPT-5.5 XHigh + PokerSkill scores $-5.68 \pm 4.14$ bb/100 after aggregating internal runs, and zero-shot GPT-5.5 XHigh scores $-9.2 \pm 2.8$ bb/100. Zero-shot baseline values should be verified against the cited GTO Wizard benchmark before submission.}
    \label{fig:gtowizard-results}
\end{figure}


==> sections/ethics.tex <==
This work studies LLM-based poker agents in a controlled research setting against GTOWizard benchmark. We do not deploy these agents on real-money platforms or against human players without their knowledge. All external services (GTOWizard, OpenAI API, Anthropic API) were used under their respective terms of service for research purposes.

\paragraph{Potential for misuse.}
Poker AI systems could in principle be used for unfair advantage in online gambling. We note that (1) our agents operate at 15--20 seconds per decision in average, making real-time deployment impractical on platforms with time limits; (2) the API costs (\$0.07--\$0.30 per hand) exceed expected winnings at most stakes; (3) our agents work in two-player settings with 200bb stacks, and can not play multi-player online poker directly; and (4) major poker platforms already employ bot-detection systems. We encourage responsible use of this research for advancing AI reasoning capabilities rather than for gambling exploitation.

\paragraph{AI assistants.}
We used Claude Code (Anthropic) to assist with experiment scripting, coding, data analysis, and LaTeX formatting during the preparation of this manuscript. All scientific claims, experimental designs, and interpretations are the authors' own. The poker skill prompts and evaluation framework were designed and validated by the authors.


==> sections/limitations.tex <==
\paragraph{Evaluation scope.}
Our evaluation is limited to heads-up no-limit Texas hold'em against a single opponent (GTOWizard). We use GTOWizard exclusively because its AIVAT variance reduction (${\sim}30\times$ vs.\ raw outcomes) enables statistically meaningful evaluation at 5{,}000 hands; without it, equivalent standard errors would require ${\sim}150{,}000$ hands per agent, exceeding \$30{,}000 per configuration at our LLM cost rates. Multiplayer poker introduces non-zero-sum dynamics, coalition effects, and opponent-specific exploitation that PokerSkill does not address. %Generalization beyond the GTO benchmark is unknown.

%\paragraph{Performance ceiling.} While the best PokerSkill agent substantially outperforms Slumbot, it still loses to GTOWizard. We do not claim GTO-level play; residual losses indicate systematic suboptimality in sizing decisions and multi-street planning that the budget system cannot fully resolve.

\paragraph{Missing ablations.}
We do not provide formal ablation experiments isolating the contribution of individual components. The cost of LLM API calls with extended reasoning (\$0.07--\$0.30 per hand) makes controlled ablations across multiple configurations economically prohibitive at statistically meaningful sample sizes. We provide indirect evidence of the LLM's contribution through cross-model performance differences, but acknowledge that a full component-wise ablation would strengthen the paper's claims.

%\paragraph{Manual calibration.} The ATT/DEF budget tables are interpretable but manually calibrated by poker experts among the authors, informed by GTO theory and solver study. While the same tables work for three architecturally different LLMs (suggesting they encode general poker principles rather than model-specific patterns), we cannot rule out some degree of benchmark-specific tuning. The budget values and skill library were finalized before the main evaluation runs; however, earlier development iterations did use GTOWizard for debugging (approximately 500 hands total across all development runs). Sensitivity analysis of budget values remains future work.

%\paragraph{Statistical power.} The cross-model comparisons (GPT-5.5 vs.\ Claude Opus 4.6 vs.\ Opus 4.7) are suggestive but not all pairwise differences reach statistical significance at current sample sizes (5{,}000 hands per configuration). The within-model improvement from default prompting to PokerSkill is large in magnitude for all models but the standard errors of the differences are also substantial due to independent evaluation samples.

%\paragraph{Classification granularity.} PokerSkill depends on the choice of labels and prompt fragments. If the hand analyzer merges two strategically different hand classes, or if the action-line analyzer treats a rare line as a common one, the prompt can give the model the wrong local rule.

%\paragraph{Residual error patterns.} Three categories of residual errors persist despite PokerSkill's scaffolding. First, \emph{sizing judgment}: the budget permits betting but the LLM selects a suboptimal size. Second, \emph{boundary ambiguity}: hands near the boundary between two classes receive slightly misaligned guidance. Third, \emph{multi-street incoherence}: per-decision budgets are locally sound but the three-street sequence is not globally planned, because the budget system lacks forward-looking search. These failure modes suggest that prompt scaffolding has inherent limits: it can constrain and guide but cannot replace the global optimization that solvers provide.

\paragraph{Cost and latency.}
Frontier LLM calls with extended reasoning are expensive (\$0.07--\$0.30/hand) and slow (15--20s per decision), limiting practical deployment to research settings rather than real-time play.

